Finding Taint-Style Vulnerabilities in Linux-based Embedded Firmware with SSE-based Alias Analysis

Although the importance of using static analysis to detect taint-style vulnerabilities in Linux-based embedded firmware is widely recognized, existing approaches are plagued by three major limitations. (a) Approaches based on symbolic execution may miss alias information and therefore suffer from a high false-negative rate. (b) Approaches based on VSA (value set analysis) often provide an over-approximate pointer range. As a result, many false positives could be produced. (c) Existing work for detecting taint-style vulnerability does not consider indirect call resolution, whereas indirect calls are frequently used in Internet-facing embedded devices. As a result, many false negatives could be produced. In this work, we propose a precise demand-driven flow-, context- and field-sensitive alias analysis approach. Based on this new approach, we also design a novel indirect call resolution scheme. Combined with sanitization rule checking, our solution discovers taint-style vulnerabilities by static taint analysis. We implemented our idea with a prototype called EmTaint and evaluated it against 35 real-world embedded firmware samples from six popular vendors. EmTaint discovered at least 192 bugs, including 41 n-day bugs and 151 0-day bugs. At least 115 CVE/PSV numbers have been allocated from a subset of the reported vulnerabilities at the time of writing. Compared to state-of-the-art tools such as KARONTE and SaTC, EmTaint found significantly more bugs on the same dataset in less time.

==> 6.Implementation.tex <==
\section{Implementation}

\subsection{Binary pre-process}

We use IDA Pro[xxx] to load binary, identify functions, and generate control flow graphs (CFG) and call graphs (CG).
Then we convert the binary into an intermediate language VEX, the IR of the Valgrind project~\cite{nethercote2007valgrind}.
Based on the VEX IR, we can support multi-architecture binary code analysis.


\paragraph{Function recognition}
In real-world binary code analysis, we found that IDA Pro could not identify some functions that were indirectly called,
and the addresses of these functions were stored in the data segment.
Therefore, we implement a simple IDA plugin to recover these functions.
We scan the data segment and collect all the “immediate” values.
If an immediate value is within the code segment interval,
and the first of the instructions from the immediate address meet the function header identity,
we recovery the function through the python APIs of IDA Pro.


\paragraph{VEX IR pre-processing}
% Neither indirect call resolution nor taint-style vulnerability check will analyze all function.
% Therefore, we do not need to convert all the functions code to IR,
% but rather to dynamically convert the function code to IR based on the data flow analysis.
We convert binary code to IR based on Angr and the CFG generated by IDA Pro.
Instead of using Angr to identify functions and generate CFG, we chose IDA Pro for the following reasons:
\begin{enumerate}[label=\arabic*)]
\item IDA Pro can better identify tail function calls and resolve most indirect jumps (e.g. switch jump).
\item In real-world code analysis, we found there are some special binaries that 
Angr could not recover the symbol table of the dynamic library function, resulting in disassembly failure.
\item IDA is more stable when the size of binary code is large.
\end{enumerate}
As described in Section~\ref{section:trace}, our data flow analysis can start with any function.
Therefore, we dynamically convert the function code into IR according to the needs of data flow analysis instead of all functions.
Then, we implement variable type recovery and loop variable analysis based on the IR.


\subsection{Data-flow implementation}
In our system, the core of data flow analysis is the symbolic expression update, which is implemented based on the module $Claripy$ from Angr.
We extend the $Claripy$ module to support $load/store$ operations, variable live-cycle tracking, loop expression structure, and more.
At the same time, we also implement the symbolic expressions merge function. 
Especially when taint analysis occurs in the case of loops and multi-path branches,
a large number of tainted variables are generated based on different paths.
We combine similar tainted variables to improve the efficiency of analysis

